A Search for Exoplanet Candidates in TESS 2-min Light Curves using Joint Bayesian Detection

In this work, we apply an exploratory joint Bayesian transit detector (Taaki et al. 2020), previously evaluated using Kepler data, to the 2 min simple aperture photometry light curve data in the continuous viewing zone for the Transiting Exoplanet Survey Satellite (TESS) over three years of observation. The detector uses Bayesian priors, adaptively estimated, to model unknown systematic noise and stellar variability incorporated in a Neyman-Pearson likelihood ratio test for a candidate transit signal; a primary goal of the algorithm is to reduce overfitting. The detector was adapted to the TESS data and refined to improve outlier rejection and suppress false alarm detections in post-processing. The statistical performance of the detector was evaluated using transit injection tests, where the joint Bayesian detector achieves an 80.0 % detection rate and a 19.1% quasi-false alarm rate at a detection threshold {\tau} = 10; this is a marginal, although not statistically significant, improvement of 0.2% over a reference sequential detrending and detection algorithm. In addition, a full search of the input TESS data was performed to evaluate the recovery rate of known TESS objects of interest (TOI) and to perform an independent search for new exoplanet candidates. The joint detector has a 73% recall rate and a 63% detection rate for known TOI; the former considers a match against all detection statistics above threshold while the latter considers only the maximum detection statistic.

==> compute.tex <==
\section{Sector-to-sector Detector} \label{sec: decompose}
% we drop the index i for brevity
%\par The matched filter detection test described in Equation \ref{eq: detector} is of computational complexity $O(|\mathbf{T}|N^2)$ due to the multiplication of the $[N \times N]$ matrix $\Cov_{\mathbf{z}_i}^{-1}$ and a length $N$ candidate transit $\mathbf{t}$ for $|\mathbf{T}|$ such candidates. 
\par A year long TESS lightcurve consists of 13 sectors of data. In our pipeline noise is modelled as independent between sectors. The noise $\mathbf{z}_i$ is described by a covariance of the form $\Cov_{\mathbf{z}_i} = \Cov_{\mathbf{s}_i} + \mathbf{V} \Cov_{\mathbf{c}} \mathbf{V}^T$. Systematics are estimated sector to sector, therefore the term $\mathbf{V} \Cov_{\mathbf{c}} \mathbf{V}^T$ admits a block diagonal structure, where each block is the covariance model $\mathbf{V}_q \Cov_{\mathbf{c}(q)} \mathbf{V}_q^T$ for a single sector $q \in Q$. A similar block diagonal structure is adopted for the stochastic noise, since a sector long model reasonably accounts for variability occurring on transit timescales. For a sector $q$ the noise covariance is of the form $\Cov_{\mathbf{z}_i(q)} =  \Cov_{\mathbf{s}_i(q)} + \mathbf{V} \Cov_{\mathbf{c}(q)} \mathbf{V}^T$. The structure of the noise covariance for all sectors is given as:
\begin{equation}
   \Cov_{\mathbf{z}_i} =  \begin{bmatrix}
    \Cov_{\mathbf{z}_i(1)} \\
    & \Cov_{\mathbf{z}_i(2)} \\
    && \ddots \\
    &&& \Cov_{\mathbf{z}_i(Q)} 
    \end{bmatrix}
\end{equation}
Due to the properties of block-diagonal matrices, the inverse covariance $\Cov_{\mathbf{z}_i}^{-1}$ also admits a block-diagonal structure and each block $\Cov_{\mathbf{z}_i}^{-1}|_{q}$ can be computed as the inverse of the corresponding sector $\Cov_{\mathbf{z}_i(q)}^{-1}$. The block diagonal structure of $\Cov_{\mathbf{z}_i}^{-1}$ allows the matched filter described in Equation \ref{eq: detector} to be decomposed across multiple sectors $q \in Q$ as:
\begin{align} \label{eq: det2}
\frac{\sum_{q \in Q} \mathbf{\hat{y}}_{i, q}^T \Cov_{\mathbf{z}_i(q)}^{-1} \bold{t}_q}{\sqrt{\sum_{q \in Q} \bold{t}_q^T \Cov_{\mathbf{z}_i(q)}^{-1} \bold{t}_q}} \LRT{H_1}{H_0} \tau
\end{align}

\par The matched filter is a normalized detector, scaling the candidate transit signal by $\alpha \in \mathbb R^+$ will not effect the detection statistic. Therefore a candidate transit depth is not needed to parameterize $\mathbf{T}$.

%In other words, for a signal $\bold{t}_{\alpha} = \alpha \bold{t}$ 
%\begin{align} \label{eq: det2}
%    \frac{\bold{y}^T\mathbf{\Cov_{z}}^{-1}\bold{t}_{\alpha}}{\sqrt{\bold{t}_{\alpha}^T \mathbf{\Cov_{z}}^{-1} \bold{t}_{\alpha}}} =    \frac{\bold{y}^T\mathbf{\Cov_{z}}^{-1}\bold{t}}{\sqrt{\bold{t}^T \mathbf{\Cov_{z}}^{-1} \bold{t}}}
%\end{align} 

However to correctly compute Equation \ref{eq: det2}, the lightcurve broken up by sector $\mathbf{\hat{y}}_{i, q}$ must be normalized so that the transit strength is constant for all sectors. In our implementation, we chose to compute detection statistics restricted per sector, and form an approximation of Equation \ref{eq: det2} with the normalized sum of these matched filters. 
%Practically this means there is no need to normalize the lightcurve $\mathbf{\hat{y}}_{i, q}$ and reduced the intermediary data output. 
\begin{align} \label{eq: final_det}
  T(\mathbf{y}_i) = \frac{1}{\sqrt{Q}} \sum_{q \in Q} \frac{ \mathbf{\hat{y}}_{i, q}^T \mathbf{\Cov}_{\mathbf{z}_i(q)}^{-1} \bold{t}_q}{\sqrt{\bold{t}_q^T \mathbf{\Cov}_{\mathbf{z}_i(q)}^{-1} \bold{t}_q}} \LRT{H_1}{H_0} \tau
\end{align}

\subsection{Computational methods and complexity} \label{sec: compute}

This section characterizes the computation of detection tests in the schematic of the pipeline in Figure \ref{fig: pipeline_overview}. 
This project was completed with $250,000$ node hour allocation, with $32$ core hours per node hour on the Blue Waters petascale system. Per year of lightcurve data detection tests required $\sim$ $50,000$ node hours, with $50$ TB of intermediate storage required. 

%In this section we drop the sector notation $q \in Q$, as the computational pattern and results described in this section can be applied regardless of whether the covariance decomposes sector-wise.
\subsubsection{Efficient computation of many transit detection tests}  \label{sec: compute_complex}
The inverse covariance calculations $\Cov_{\mathbf{z}}^{-1}$ are not a significant part of the pipeline computations as they only need to be performed once per lightcurve since the covariance is independent of the transit $\bold{t}$ under study.  \\
The detector involves the computation of a matrix-vector product $\Cov_{\mathbf{z}}^{-1} \mathbf{t}$ of $O(N^2)$  which is reused in the numerator and denominator of a transit detection test. We efficiently implement the computation of many of these calculations for a large number of candidate transit signals $\mathbf{t} \in \mathbf{T}$ by exploiting similarities between transit signals of fixed duration $d$, a similar approach is described in \citep{jenkins_2010}. Candidate transit signals are represented by a signal that is zero everywhere except on disjoint in-transit cadences. As such a candidate transit signal may be decomposed into a number of disjoint single transit events. The computation $\Cov_{\mathbf{z}}^{-1} \mathbf{t}$ can be decomposed into the sum of matrix vector products of $\Cov_{\mathbf{z}}^{-1}$ with single transit events comprising $\mathbf{t}$. The matrix-vector product of $\Cov_{\mathbf{z}}^{-1}$ with a single transit event can then be efficiently computed, since the entries of $\Cov_{\mathbf{z}}^{-1}$ needed for this computation represent a contiguous slice of matrix columns in memory, the $d$ columns of length $N$ are then summed to produce a length $N$ vector, hence this computation consists of $d N$ additions. These calculated vectors for single transit events are stored to compute detection tests for a range of candidate transit signals of fixed transit duration $d$, hence performing $d N$ adds $\frac{N}{\delta e}$ times, therefore to compute the single transit calculations for fixed duration $d$ requires $\frac{N^2 d}{\delta e}$ additions. Computing these values for all candidate durations $D$ therefore requires $\sum_{d \in D} \frac{N^2 d}{\delta e}$ additions. \\

Denote the average number of transit events for $\mathbf{t} \in \mathbf{T}$ as $\mu_{\mathbf{t}}$. Matrix-vector products $\Cov_{\mathbf{z}}^{-1} \mathbf{t}$ on average require the addition of $\mu_{\mathbf{t}}$ single transit vectors of length $N$ per transit. Therefore requiring $|\mathbf{T}|N \mu_{\mathbf{t}}$ additions for transit search space $\mathbf{T}$. The average number of transit events $\mu_t$ in a transit signal $\mathbf{t}$ is a constant factor, see Appendix section \ref{ap: mu_t} for this calculation. \\
%\JTnote{This computation occurs once per transit, add number of transit events $\#_t$ length $N_q$ vectors $O(\#_{\mathbf{t}}N_q)$ due to the periodicity of the transit signal just select the $\#_t$ columns to add. The output of which is a length $N_q$ vectors and then inner product with $y$, $O(N_q)$, final complexity per sector $O(|T|_q ((1+\#_{\mathbf{t}})N_q ) +  \frac{\sum_{d} d N_q^2}{\delta e})$. The leading order $O(|T|_q \#_{\mathbf{t}}N_q)$, we note that for our transit search space, first $ log (N_q) > \#_{\mathbf{t}} \sim 2-3$. }

A final detection test for a single candidate transit $\mathbf{t}$ requires inner product calculations of $\Cov_{\mathbf{z}}^{-1} \mathbf{t}$ with $\mathbf{y}$ in the numerator, and $\mathbf{t}$ in the denominator. This requires $N$ multiplications and additions respectively. The transit search of $\mathbf{T}$ for a single lightcurve is of complexity $O(|\mathbf{T}| N (1 + \mu_{\mathbf{t}} ) + \frac{\sum_{d \in D}d N^2}{\delta_e} )$. The size of the transit-search space $|\mathbf{T}| \gg N$, therefore we can drop the last term in the complexity. Since $\mu_t$ is constant factor, the complexity is therefore $O(|\mathbf{T}| N)$. 

%In principle the achievable complexity is further reduced to $O(|\mathbf{T}|(N + N_q\mu_{\mathbf{t}}) +  \frac{\sum_{d \in D}d N N_q}{\delta_e})$ due to the sector-wise decomposition. However, we compute excess transit \\

%\par After detection statistics are computed for each sector for the restriction of the transit search space to that sector $\mathbf{T}|_q$, statistics are then combined to produce Equation \ref{eq: final_det} with a windowed search for the maximizing statistic over $|\mathbf{T}|_{q, d, P}$ subject to an epoch window of $2 [h]$. Due to the sets $\mathbf{T}|_q$ being distinct, obtaining the relevant sector-wise statistics to compute the detector for a particular $\mathbf{t}$ is a computationally challenging indexing problem. 

\subsubsection{High-performance-computing pipeline}
Lightcurve SAP data as provided by the MAST archive is broken down per lightcurve, per sector of data. Each file is of size 1.5 MB, a year of data for lightcurves from the continuous viewing zone occupies $\sim$ 50 GB in hard disk. Computations as described in Section \ref{sec: compute_complex} are performed per sector, before combined as in Equation \ref{eq: final_det} to compute detection tests for each lightcurve, over the set of transits $\bold{T}$ for a full year. Computations described in this section, are independent between lightcurves, and between candidate transit durations. We describe the pipeline to implement the computation of detection tests for a year-long lightcurve on the Blue Waters petascale system \citep{MENDES2015327} with full node utilization, and the associated computational requirements. \\

In the first step, per lightcurve, per sector, the inverse covariance $\Cov_{\mathbf{z}_i(q)}^{-1}$ of size  $N_q \times N_q$ is computed once per lightcurve. This matrix is $\sim$ 1.7 GB and stored on hard disk, to store covariances for all sectors (13) within a year requires 22 GB per lightcurve. For all lightcurves in the CVZ of a single year requires approximately 35 TB. \\

A Bluewaters XE node consists of 32 CPU cores with 32 GB of local memory. The unit of parallelism is a task, with one task requiring a single CPU core, and 20 placed per XE node. A task corresponds to the computation of a complete set of detection tests of fixed duration $d$ and restricted to a  28-day sector, $|\mathbf{T}| _{d, N_q}| \approx 10^7$.
%, thereby including single-transit event statistics of fixed duration $d$.
The detection tests are computed as described in Section \ref{sec: compute_complex}. Each task is highly parallel, no communication is needed between tasks. The approximate number and type of major arithmetic computations for a task are summarized in Table \ref{tab:arithmetic} for the transit search space in Table \ref{tab:search_space}. \\

\begin{deluxetable}{cc}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
\tablecaption{Major Arithmetic Operations per Task \label{tab:arithmetic}}
\tablehead{
\colhead{Computation Type} & \colhead{Per task for transit Duration $d$} 
}
\startdata
Single transit calculations (additions) & $\frac{N_q^2 \cdot d}{\delta e}   \approx 10^{10}$  \\
%& $\displaystyle\prod_{d \in D }S_{d} \approx 10^{11}$  \\
Transit detection (multiplications and additions) & $ (1+\mu_{\mathbf{t}}) \cdot N_q \cdot |\mathbf{T}|_{d, N_q}| \approx 10^{11}$\\
%& $\displaystyle\prod_{d \in D }M_{d}\approx 10^{12}$ \\
\enddata
\tablecomments{1) $ \mathbf{T}|_{d, N_q} $ is the restriction of the transit search space $\mathbf{T}$ to fixed duration $d$ and length $N_q$; of size $ |\mathbf{T}|_{d, N_q}| \sim 10^7$
2) A task is the the computation of a complete set of transit detection tests of fixed duration for a single lightcurve in a 28-day TESS data segment. Numerical values computed for $d \sim 300$ LC samples. Note: $\log (N_q) > \mu_{\mathbf{t}} \sim 3$. }
\end{deluxetable} 

Since $\Cov_{\mathbf{z}_i}^{-1} \sim $ 1.7 GB, loading this full covariance for each task will hit a memory bottleneck when run in parallel. Hence we allocate tasks pertaining to the same lightcurve within a node, and load $\Cov_{\mathbf{z}_i}^{-1}$ as a memory mapped object shared between the tasks. Within a task, single transit event statistics of the form $\Cov_{\mathbf{z}_i}^{-1} \mathbf{t}_{d, s}$ are computed serially, only the $N_q \cdot D$ elements of the covariance matrix which are relevant to the single transit event $\mathbf{t}_{d, s}$ are read into local memory at a time. \\

The memory required to hold all single transit calculations per task is  $\frac{N_q^2}{\delta e}$ float 32 values, of total size $\sim$ 0.4 GB. All possible transit detection tests are output per sector, alongside the single transit detection tests.  \\

The output of the detection tests is $|\mathbf{T}|_{d, N_q}| \approx 10^7$ float32 values, of total size 18 MB (therefore $10^7$ writes per task). The individual detection results are intermediate as they are combined to form composite detection statistics as described below. Memory and I/O requirements (remote and local) per task are summarized in Table \ref{tab:resources per process}.\\

\begin{deluxetable}{cc}
\tabletypesize{\footnotesize}
\tablewidth{0pt}
\tablecaption{Memory Resources Per Task \label{tab:resources per process}}
\tablehead{
\colhead{Resource Type} & \colhead{Resources per Task} 
}
\startdata
Total Remote Disk Access (read)  & 1.7 GB \\
Total Remote Disk Access (write)  & 18 MB \\
Read Count & 2\\
Write Count & $10^7$\\
Local Memory  & 0.4 GB   \\
\enddata
\end{deluxetable}

Each task corresponding to a sector must be complete (13 tasks per 1-year lightcurve) before they can be combined to compute detection tests corresponding to a year of data. The intermediate data output associated with a complete year, for all candidate durations, is of size $|\mathbf{T}|_{d, N_q} D Q |Y|\cdot32\sim$ 15 TB. The detection tests are output for the full year for $\mathbf{T}$, requiring 1 GB per lightcurve.

